Improving the Reasoning of Multi-Image Grounding in MLLMs via Reinforcement Learning

Multimodal Large Language Models (MLLMs) perform well in single-image visual grounding but struggle with real-world tasks that demand cross-image reasoning and multi-modal instructions. To address this, we adopt a reinforcement learning (RL) based post-training strategy for MLLMs in multi-image grounding tasks. We first synthesize high-quality chain-of-thought (CoT) data for cold-start initialization, followed by supervised fine-tuning (SFT) using low-rank adaptation (LoRA). Subsequently, we apply rejection sampling with the merged SFT model to curate reliable RL data and use rule-based RL to guide the model toward optimal reasoning paths. Extensive experiments demonstrate the effectiveness of our approach, achieving +9.04% on MIG-Bench and +4.41% on average across seven out-of-domain benchmarks.

==> sec/2_related_works.tex <==
\section{Related Works}

\subsection{MLLM-based Referring Grounding.}

Referring grounding, also known as referring expression comprehension (REC), involves identifying a specific object within an image based on a given natural language referring expression. 
With the rapid advancement of multimodal large language models (MLLMs)~\cite{liu2023visual,wang2024qwen2,li2024llava,jiang2024mantis,li2024llavainterleave,bai2025qwen2,zhu2025internvl3}, significant progress has been made in extending their capabilities to address more challenging tasks, including fine-grained image understanding~\cite{wang2024advancing}, object detection~\cite{zhan2024griffon, jiao2024lumen}, and visual grounding~\cite{lai2024lisa,yan2024visa,rasheed2024glamm,li2024groundinggpt}.
Although these MLLMs have achieved strong performance on standard benchmarks such as RefCOCO/+/g~\cite{mao2016generation,yu2016modeling}, their visual grounding capabilities remain largely confined to single-image contexts and face substantial difficulties in capturing cross-image relationships.
Recent efforts, such as Migician~\cite{li2025migician}, introduce multi-image grounding tasks and further propose a two-stage SFT strategy, achieving notable results in these tasks. 
However, such approaches still exhibit insufficient reasoning abilities and limited generalization in multi-image and out-of-domain settings. 
In this paper, we explore the potential of the RL paradigm to improve the reasoning and comprehension abilities of MLLMs in multi-image grounding scenarios.

\subsection{RL-based Reasoning Model}

% The remarkable success of large language models
Recent advancements in improving the reasoning ability of large language models~\cite{jaech2024openai,xu2024llava,el2025competitive,guo2025deepseek,team2025kimi} have been made through CoT-based or RL-based post-training.
Previous methods, such as Reinforcement Learning from Human Feedback (RLHF)~\cite{ouyang2022training} and Direct Preference Optimization (DPO)~\cite{rafailov2023direct}, have explored aligning models with human preferences, achieving remarkable success in enhancing reasoning and instruction-following capabilities.
Recently, DeepSeek-R1~\cite{guo2025deepseek} employes the GRPO~\cite{shao2024deepseekmath} algorithm as a post-training method without the need for critic models, demonstrating the potential of large-scale reinforcement learning.
Inspired by the success of DeepSeek-R1, a series of subsequent works rapidly adopt this approach to enhance multi-modal reasoning across various domains, including mathematical problem solving~\cite{yang2025r1,peng2025skywork,huang2025vision,zhang2025r1,deng2025openvlthinker}, video understanding~\cite{feng2025video,zhang2025tinyllava,liao2025improved,wang2025time}, and visual perception tasks~\cite{shen2025vlm,liu2025seg,deng2025boosting,liu2025visual,zhan2025vision,yu2025perception,tan2025reason}.
Among the most closely related works to ours, VLM-R1~\cite{shen2025vlm}, Visual-RFT~\cite{liu2025visual}, Vision-R1~\cite{zhan2025vision}, and Perception-R1~\cite{yu2025perception}, primarily focus on single-image visual grounding or object detection. 
However, these approaches lack the capability for multi-image perception and reasoning.
In this paper, we follow the DeepSeek-R1 paradigm and extend it to the multi-image grounding tasks, while also achieving strong performance on both multi-image grounding and multi-image understanding tasks.




